Rethinking HTG Evaluation: Bridging Generation and Recognition

The evaluation of generative models for natural image tasks has been extensively studied. Similar protocols and metrics are used in cases with unique particularities, such as Handwriting Generation, even if they might not be completely appropriate. In this work, we introduce three measures tailored for HTG evaluation, $ \text{HTG}_{\text{HTR}} $, $ \text{HTG}_{\text{style}} $, and $ \text{HTG}_{\text{OOV}} $, and argue that they are more expedient to evaluate the quality of generated handwritten images. The metrics rely on the recognition error/accuracy of Handwriting Text Recognition and Writer Identification models and emphasize writing style, textual content, and diversity as the main aspects that adhere to the content of handwritten images. We conduct comprehensive experiments on the IAM handwriting database, showcasing that widely used metrics such as FID fail to properly quantify the diversity and the practical utility of generated handwriting samples. Our findings show that our metrics are richer in information and underscore the necessity of standardized evaluation protocols in HTG. The proposed metrics provide a more robust and informative protocol for assessing HTG quality, contributing to improved performance in HTR. Code for the evaluation protocol is available at: https://github.com/koninik/HTG_evaluation.

==> sections/9_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented an evaluation protocol to examine the generation quality in Handwritten Text Generation systems. 
We propose HTG\textsubscript{HTR}, HTG\textsubscript{style}, and HTG\textsubscript{OOV} to evaluate the variance, the style imitation, and the successful content generation of synthetic data using HTG systems.
The protocol can serve as a standard guideline for future research to establish a standardized process to evaluate synthetic handwritten text samples depending on the dataset needs.
We presented an evaluation protocol to examine the generation quality in Handwritten Text Generation systems. 

